Metadata Archaeology: Unearthing Data Subsets by Leveraging Training Dynamics

Modern machine learning research relies on relatively few carefully curated datasets. Even in these datasets, and typically in `untidy' or raw data, practitioners are faced with significant issues of data quality and diversity which can be prohibitively labor intensive to address. Existing methods for dealing with these challenges tend to make strong assumptions about the particular issues at play, and often require a priori knowledge or metadata such as domain labels. Our work is orthogonal to these methods: we instead focus on providing a unified and efficient framework for Metadata Archaeology -- uncovering and inferring metadata of examples in a dataset. We curate different subsets of data that might exist in a dataset (e.g. mislabeled, atypical, or out-of-distribution examples) using simple transformations, and leverage differences in learning dynamics between these probe suites to infer metadata of interest. Our method is on par with far more sophisticated mitigation methods across different tasks: identifying and correcting mislabeled examples, classifying minority-group samples, prioritizing points relevant for training and enabling scalable human auditing of relevant examples.

==> figure_imagenet_random_outputs.tex <==
    




\begin{figure*}[!t]\centering
    \begin{subfigure}[b]{\textwidth}
         \centering
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/digital_watch/all_mislabeled/rank_0_idx_682036_count_1_conf_0.80_digital watch_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/digital_watch/all_mislabeled/rank_0_idx_682039_count_4_conf_0.50_digital watch_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/digital_watch/all_mislabeled/rank_0_idx_682051_count_9_conf_0.50_digital watch_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/digital_watch/all_mislabeled/rank_0_idx_682103_count_6_conf_0.80_digital watch_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/digital_watch/all_mislabeled/rank_0_idx_682171_count_0_conf_0.85_digital watch_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/digital_watch/all_mislabeled/rank_0_idx_682180_count_7_conf_0.60_digital watch_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/digital_watch/all_mislabeled/rank_0_idx_682199_count_3_conf_0.95_digital watch_random_outputs.png} \\ \vspace{1mm}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/digital_watch/all_mislabeled/rank_0_idx_682216_count_5_conf_0.55_digital watch_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/digital_watch/all_mislabeled/rank_0_idx_682235_count_8_conf_0.50_digital watch_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/digital_watch/all_mislabeled/rank_0_idx_682242_count_11_conf_0.60_digital watch_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/digital_watch/all_mislabeled/rank_0_idx_682243_count_10_conf_0.90_digital watch_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/digital_watch/all_mislabeled/rank_0_idx_682264_count_12_conf_0.85_digital watch_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/digital_watch/all_mislabeled/rank_0_idx_682282_count_2_conf_0.85_digital watch_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/digital_watch/all_mislabeled/rank_0_idx_682687_count_13_conf_0.90_digital watch_random_outputs.png}
        
        \caption{Digital Watch}
    \end{subfigure}
    
    
    
    \begin{subfigure}[b]{\textwidth}
         \centering
         
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/plastic_bag/all_mislabeled/rank_0_idx_932959_count_2_conf_0.55_plastic bag_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/plastic_bag/all_mislabeled/rank_0_idx_932965_count_4_conf_0.90_plastic bag_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/plastic_bag/all_mislabeled/rank_0_idx_932986_count_6_conf_0.60_plastic bag_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/plastic_bag/all_mislabeled/rank_0_idx_933071_count_0_conf_0.55_plastic bag_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/plastic_bag/all_mislabeled/rank_0_idx_933085_count_10_conf_0.50_plastic bag_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/plastic_bag/all_mislabeled/rank_0_idx_933306_count_1_conf_0.75_plastic bag_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/plastic_bag/all_mislabeled/rank_0_idx_933336_count_3_conf_0.55_plastic bag_random_outputs.png} \\ \vspace{1mm}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/plastic_bag/all_mislabeled/rank_0_idx_933442_count_5_conf_0.50_plastic bag_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/plastic_bag/all_mislabeled/rank_0_idx_933503_count_9_conf_0.55_plastic bag_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/plastic_bag/all_mislabeled/rank_0_idx_933952_count_8_conf_0.60_plastic bag_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/plastic_bag/all_mislabeled/rank_0_idx_933962_count_7_conf_0.55_plastic bag_random_outputs.png}
    
        \caption{Plastic Bag}
    \end{subfigure}
    
    \begin{subfigure}[b]{\textwidth}
         \centering
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/toilet_tissue/all_mislabeled/rank_0_idx_1280081_count_7_conf_0.55_toilet tissue_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/toilet_tissue/all_mislabeled/rank_0_idx_1280600_count_10_conf_0.50_toilet tissue_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/toilet_tissue/all_mislabeled/rank_0_idx_1280651_count_8_conf_0.65_toilet tissue_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/toilet_tissue/all_mislabeled/rank_0_idx_1280657_count_3_conf_0.80_toilet tissue_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/toilet_tissue/all_mislabeled/rank_0_idx_1280710_count_6_conf_0.75_toilet tissue_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/toilet_tissue/all_mislabeled/rank_0_idx_1280719_count_1_conf_0.85_toilet tissue_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/toilet_tissue/all_mislabeled/rank_0_idx_1280766_count_4_conf_1.00_toilet tissue_random_outputs.png} \\ \vspace{1mm}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/toilet_tissue/all_mislabeled/rank_0_idx_1280777_count_0_conf_1.00_toilet tissue_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/toilet_tissue/all_mislabeled/rank_0_idx_1280879_count_9_conf_0.85_toilet tissue_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/toilet_tissue/all_mislabeled/rank_0_idx_1280963_count_5_conf_1.00_toilet tissue_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/toilet_tissue/all_mislabeled/rank_0_idx_1281043_count_2_conf_0.90_toilet tissue_random_outputs.png}
    
        \caption{Toilet Tissue}
    \end{subfigure}
    
    \begin{subfigure}[b]{\textwidth}
         \centering
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/whiskey_jug/all_mislabeled/rank_0_idx_1153656_count_6_conf_1.00_whiskey jug_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/whiskey_jug/all_mislabeled/rank_0_idx_1153748_count_5_conf_0.95_whiskey jug_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/whiskey_jug/all_mislabeled/rank_0_idx_1153873_count_0_conf_0.55_whiskey jug_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/whiskey_jug/all_mislabeled/rank_0_idx_1153933_count_7_conf_0.75_whiskey jug_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/whiskey_jug/all_mislabeled/rank_0_idx_1154049_count_4_conf_0.85_whiskey jug_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/whiskey_jug/all_mislabeled/rank_0_idx_1154058_count_2_conf_0.80_whiskey jug_random_outputs.png}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/whiskey_jug/all_mislabeled/rank_0_idx_1154105_count_1_conf_0.45_whiskey jug_random_outputs.png} \\ \vspace{1mm}
        \includegraphics[width=\smallfigsize\linewidth]{Figures/loss_traj/surfacing/imagenet/ex_surfaced/whiskey_jug/all_mislabeled/rank_0_idx_1154270_count_3_conf_0.95_whiskey jug_random_outputs.png}
        
        \caption{Whiskey Jug}
    \end{subfigure}
    \caption{All examples surfaced through the use of \textit{MAP-D} on ImageNet train set from the random outputs category for four different classes. Sub-caption refers to the ground truth class.}
    \label{fig:surfaced_examples_imagenet_random_outputs}
\end{figure*}

==> figure_imagenet_val.tex <==
\begin{figure*}[!t]\centering
    \begin{tikzpicture}[x=130pt,y=-60pt,
            head/.style={font=\footnotesize,execute at begin node={\strut},execute at end node={\strut}},
            cn/.style={head,text width=65pt,align=center,draw,rectangle,rounded corners=3pt,inner xsep=1pt,inner ysep=0.25pt,fill=white,draw=black!50},
            rn/.style={head,text width=35pt,inner sep=5pt,align=right},
            img/.style={inner sep=0.5pt,yshift=25pt},
            L/.style={img,anchor=north east},
            R/.style={img,anchor=north west},
        ]
        \def\colimg#1{\includegraphics[width=0.12\linewidth]{Figures/surfaced_examples/#1}}
            \node[rn] (r1) at (0.38,1) {Typical};
            \node[rn] (r2) at (0.38,2) {Atypical};
            \node[rn] (r3) at (0.38,3) {Corrupted};
            \node[rn] (r4) at (0.38,4) {Random\\ Output};
            \node[cn] (c1) at (1,0.4) {Digital Watch};
            \node[cn] (c2) at (2,0.4) {Plastic Bag};
            \node[cn] (c3) at (3,0.4) {Toilet Tissue};
            \node[L] (e-1-1) at (r1-|c1.south) {\colimg{typical/rank_0_11546_digital watch.png}};
            \node[R] (e-2-1) at (r1-|c1.south) {\colimg{typical/rank_0_11547_digital watch.png}};
            \node[L] (e-3-1) at (r1-|c2.south) {\colimg{typical/rank_0_15108_plastic bag.png}};
            \node[R] (e-4-1) at (r1-|c2.south) {\colimg{typical/rank_0_15109_plastic bag.png}};
            \node[L] (e-5-1) at (r1-|c3.south) {\colimg{typical/rank_0_20182_toilet tissue.png}};
            \node[R] (e-6-1) at (r1-|c3.south) {\colimg{typical/rank_0_20183_toilet tissue.png}};
            \node[L] (e-1-2) at (r2-|c1.south) {\colimg{atypical/rank_0_10947_digital watch.png}};
            \node[R] (e-2-2) at (r2-|c1.south) {\colimg{atypical/rank_0_10948_digital watch.png}};
            \node[L] (e-3-2) at (r2-|c2.south) {\colimg{atypical/rank_0_14969_plastic bag.png}};
            \node[R] (e-4-2) at (r2-|c2.south) {\colimg{atypical/rank_0_14970_plastic bag.png}};
            \node[L] (e-5-2) at (r2-|c3.south) {\colimg{atypical/rank_0_20418_toilet tissue.png}};
            \node[R] (e-6-2) at (r2-|c3.south) {\colimg{atypical/rank_0_20419_toilet tissue.png}};
            \node[L] (e-1-3) at (r3-|c1.south) {\colimg{corrupted/rank_0_3781_digital watch.png}};
            \node[R] (e-2-3) at (r3-|c1.south) {\colimg{corrupted/rank_0_3783_digital watch.png}};
            \node[L] (e-3-3) at (r3-|c2.south) {\colimg{corrupted/rank_0_5922_plastic bag.png}};
            \node[R] (e-4-3) at (r3-|c2.south) {\colimg{corrupted/rank_0_5923_plastic bag.png}};
            \node[L] (e-5-3) at (r3-|c3.south) {\colimg{corrupted/rank_0_8759_toilet tissue.png}};
            \node[R] (e-6-3) at (r3-|c3.south) {\colimg{corrupted/rank_0_8760_toilet tissue.png}};
            \node[L] (e-1-4) at (r4-|c1.south) {\colimg{random_outputs/rank_0_277_digital watch.png}};
            \node[R] (e-2-4) at (r4-|c1.south) {\colimg{random_outputs/rank_0_276_digital watch.png}};
            \node[L] (e-3-4) at (r4-|c2.south) {\colimg{random_outputs/rank_0_403_plastic bag.png}};
            \node[R] (e-4-4) at (r4-|c2.south) {\colimg{random_outputs/rank_0_407_plastic bag.png}};
            \node[L] (e-5-4) at (r4-|c3.south) {\colimg{random_outputs/rank_0_594_toilet tissue.png}};
            \node[R] (e-6-4) at (r4-|c3.south) {\colimg{random_outputs/rank_0_595_toilet tissue.png}};
            \begin{scope}[on background layer,rounded corners=2pt]
                \draw[black!50] ([shift={(-2pt,0pt)}]c1.west-|e-1-1.west) rectangle ([shift={(2pt,-2pt)}]e-2-4.south east);
                \draw[black!50] ([shift={(-2pt,0pt)}]c2.west-|e-3-1.west) rectangle ([shift={(2pt,-2pt)}]e-4-4.south east);
                \draw[black!50] ([shift={(-2pt,0pt)}]c3.west-|e-5-1.west) rectangle ([shift={(2pt,-2pt)}]e-6-4.south east);
                \coordinate (R1) at ($(e-1-1.south)!0.5!(e-1-2.north)$);
                \coordinate (R2) at ($(e-1-2.south)!0.5!(e-1-3.north)$);
                \coordinate (R3) at ($(e-1-3.south)!0.5!(e-1-4.north)$);
                \draw[dashed,black!50] (R1-|r1.west)--([xshift=2pt]R1-|e-6-1.east);
                \draw[dashed,black!50] (R2-|r1.west)--([xshift=2pt]R2-|e-6-1.east);
                \draw[dashed,black!50] (R3-|r1.west)--([xshift=2pt]R3-|e-6-1.east);
            \end{scope}
    \end{tikzpicture}
    \caption{Examples surfaced through the use of \textit{MAP-D} on ImageNet from four different categories. Column title refer to ground truth class, row title refers to the \textit{MAP-D} curated subset used to surface. \sas{Will replace with training set images instead of validation set images and include those samples for CIFAR-10/100 within the next couple of days.}}
    \label{fig:surfaced_examples_imagenet}
\end{figure*}
